Toward Fairness via Maximum Mean Discrepancy Regularization on Logits Space

Fairness has become increasingly pivotal in machine learning for high-risk applications such as machine learning in healthcare and facial recognition. However, we see the deficiency in the previous logits space constraint methods. Therefore, we propose a novel framework, Logits-MMD, that achieves the fairness condition by imposing constraints on output logits with Maximum Mean Discrepancy. Moreover, quantitative analysis and experimental results show that our framework has a better property that outperforms previous methods and achieves state-of-the-art on two facial recognition datasets and one animal dataset. Finally, we show experimental results and demonstrate that our debias approach achieves the fairness condition effectively.

==> Motivation.tex <==
% We have identified a major shortcoming in the previous logits space regularization methods, namely the \emph{Gaussian Assumption} (GA) and \emph{Histogram Approximation} (HA) proposed by \cite{chen2020towards}. Similar to the EO objective discussed in Sec. \ref{subsec:method_fairness_criterion}, \cite{chen2020towards} used equation (\ref{eq.CV_EO}) to evaluate the fairness condition and trained a classifier that was invariant to the decision threshold using GA and HA. However, we argue that these two methods were inconsistent with the EO condition. Therefore, we have opted to use the MMD method, which possesses a strong theoretical foundation that aligns the training objectives with the EO condition.

We see a huge deficiency in the previous logits space regularization methods \emph{Gaussian Assumption} (GA) and \emph{Histogram Approximation} (HA) proposed by \cite{chen2020towards}. Same as the EO in Sec. \ref{subsec:method_fairness_criterion}, \cite{chen2020towards} evaluated the fairness condition by equation (\ref{eq.CV_EO}) and trained a classifier that was invariant to the decision threshold by GA and HA. Nonetheless, we claim that the two proposed methods were inconsistent with the EO definition. As a result, we leverage the power of MMD, which has a good theoretical property that aligns the training objectives with the equalized odds condition.

% We saw a huge deficiency in the previous logits space regularization methods \emph{Gaussian Assumption} (GA) and \emph{Histogram Approximation} (HA) proposed by \cite{chen2020towards}. Same as  $\Delta EO$ criterion in section \ref{subsec:method_fairness_criterion}, \cite{chen2020towards} evaluates the fairness condition by equation (\ref{eq.CV_EO}) and trains a fair classifier that is invariant to the decision threshold. Moreover, \cite{chen2020towards} minimizes the distance of logits distribution, same as our strategy in (\ref{eq.logit_MMD_regularization}) via GA and HA. Nonetheless, we claim that the two proposed methods are inconsistent with  $\Delta EO$ criterion. 

\textbf{Gaussian Assumption} modeled the output logits with Gaussian distributions. That is, the method assumed that optimally $l_{a^i, y} $ and $ l_{a^j, y}$, $\forall y \in \{0, 1\}$, $\forall a^i,a^j \in A$ followed the same Gaussian distributions. Moreover, GA minimized the distance of two Gaussian distributions via symmetric \emph{Kullback–Leibler} divergence, and the detailed implementation can be found in \cite{chen2020towards}. Nevertheless, since there is no clue about the logits distribution, it is not rational to assume the optimal distributions will obey the same Gaussian. As a result, the assumption limits the model's capability of fitting the optimal distribution. 

\textbf{Histogram Approximation} used an N-bins histogram to approximate confidence score distribution. To obtain a differentiable histogram, HA leveraged the Gaussian kernel to approximate the number of samples in each bin and built the distribution of the confidence score by normalizing the item frequency in each bin. Similar to GA, HA minimized the distance of the approximated histogram, i.e., $l_{a^i, y} $ and $ l_{a^j, y}$, $ \ \forall y \in \{0, 1\}$, $\forall a^i,a^j \in A$, by symmetric \emph{Kullback–Leibler} divergence. The detailed setting can be found in \cite{chen2020towards}. Nonetheless, the histogram approximation has the main drawback. \cite{silverman2018density} proved that the optimal bin size depends on the value of density in the bin and the number of sampled data points; therefore, there is no reliable algorithm to construct a histogram, and poor binning will lead to a considerable estimation error in HA.

The above analysis of the drawbacks motivates us to propose a new objective consistent with the EO. Moreover, the experiments in Sec. \ref{subsec:Results} demonstrate that our new objective function vastly outperforms GA and HA.


%  The binning process quantizes the value of the confidence score and leads to the same value in each bin; thus, it has different values at different points inside a given bin. Moreover,
